A Tensor-Train Decomposition based Compression of LLMs on Group Vector Systolic Accelerator

Large language models (LLMs) are both storage-intensive and computation-intensive, posing significant challenges when deployed on resource-constrained hardware. As linear layers in LLMs are mainly resource consuming parts, this paper develops a tensor-train decomposition (TTD) for LLMs with a further hardware implementation on FPGA. TTD compression is applied to the linear layers in ChatGLM3-6B and LLaMA2-7B models with compression ratios (CRs) for the whole network 1.94$\times$ and 1.60$\times$, respectively. The compressed LLMs are further implemented on FPGA hardware within a highly efficient group vector systolic array (GVSA) architecture, which has DSP-shared parallel vector PEs for TTD inference, as well as optimized data communication in the accelerator. Experimental results show that the corresponding TTD based LLM accelerator implemented on FPGA achieves 1.45$\times$ and 1.57$\times$ reduction in first token delay for ChatGLM3-6B and LLaMA2-7B models, respectively.

==> LLM_delay_V80.tex <==
\begin{table}[t]
\caption{TTD compressed ChatGLM3-6B and LLaMA2-7B on V80}
\centering

\resizebox{\linewidth}{!}{

\begin{tabular}{|c|cc|c|c|}
\hline
\textbf{LLMs}                                                            & \multicolumn{2}{c|}{\textbf{Operations}}                             & \textbf{\begin{tabular}[c]{@{}c@{}}GLM\\ Delay(us)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}LLaMA\\ Delay(us)\end{tabular}} \\ \hline
\multirow{14}{*}{Block}                                                  & \multicolumn{1}{c|}{\multirow{9}{*}{MHA}} & LN                       & 11.39                                                            & 12.57                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & Linear-BN(QK)            & 51.03                                                            & 91.23                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & EMB(Q)                   & 6.54                                                             & 4.82                                                               \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & EMB(K)                   & 6.80                                                             & 6.80                                                               \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & Linear-TRP               & 8.24                                                             & 47.35                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & Softmax                  & 26.08                                                            & 22.35                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & Linear-BN(V)             & 7.47                                                             & 51.94                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & Linear                   & 8.99                                                             & 44.13                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & \textbf{TTDLinear-BNRes} & \textbf{29.32}                                                   & \textbf{29.34}                                                     \\ \cline{2-5} 
                                                                         & \multicolumn{1}{c|}{\multirow{5}{*}{MLP}} & LN                       & 11.63                                                            & 11.00                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & \textbf{TTDLinear-BN}    & \textbf{43.04}                                                   & \textbf{27.03}                                                     \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & ACT                      & 21.87                                                            & 12.43                                                              \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & \textbf{TTDLinear-BNRes} & \textbf{43.49}                                                   & \textbf{27.74}                                                     \\ \cline{3-5} 
                                                                         & \multicolumn{1}{c|}{}                     & \textbf{TTDLinear-BNRes} & \textbf{37.22}                                                   & \textbf{24.73}                                                     \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Output\\ Layers\end{tabular}} & \multicolumn{2}{c|}{LN}                                              & 13.78                                                            & 12.28                                                              \\ \cline{2-5} 
                                                                         & \multicolumn{2}{c|}{Linear-BNArgmax}                                 & 701.18                                                           & 349.16                                                             \\ \hline \hline
\multirow{2}{*}{\textbf{Summary}}                                        & \multicolumn{2}{c|}{\textbf{First Token Delay(ms)}}                  & \textbf{14.34}                                                   & \textbf{15.20}                                                     \\ \cline{2-5} 
                                                                         & \multicolumn{2}{c|}{\textbf{Peak Speed(token/s)}}                    & \multicolumn{1}{l|}{\textbf{69.7(1.45$\times$)}}                 & \multicolumn{1}{l|}{\textbf{65.8(1.57$\times$)}}                   \\ \hline
\end{tabular}

}

\end{table}
